Compositional Verification and Optimization of Interactive Markov Chains

Interactive Markov chains (IMC) are compositional behavioural models extending labelled transition systems and continuous-time Markov chains. We provide a framework and algorithms for compositional verification and optimization of IMC with respect to time-bounded properties. Firstly, we give a specification formalism for IMC. Secondly, given a time-bounded property, an IMC component and the assumption that its unknown environment satisfies a given specification, we synthesize a scheduler for the component optimizing the probability that the property is satisfied in any such environment.

==> cegames-direct.tex <==
% $Id: cegames.tex 341 2012-10-09 13:11:50Z xkretins $

\section{Controller-Environment Games}\label{sec:ceg}


In this section, we want to reduce our problem into a two-player \emph{controller--environment game} (CE game) $\game$. 
Here player $\playercon$ controls the decisions over internal transitions in $\imc$;  player $\playerenv$ simulates the environment, i.e.~decides where synchronization can occur and \emph{when}. Thus the stochastic flow of time of the environment (limited in an unknown way) is now replaced by a free \emph{non-deterministic} choice of the player, which allows for game solving techniques.

In essence, $\playercon$ chooses in each state with internal transitions one of
them, and $\playerenv$ chooses in each state with external (and hence
synchronizing) transitions either which of them should be taken, or a \emph{delay} $t_\ext \in \Rsetp$.
The internal and external transitions take zero time to be executed once chosen. If no
zero time transition is chosen, the delay $t_\ext$ determined by $\playerenv$ competes with the
Markovian transitions. Further, $\playerenv$ is limited which actions he can choose by the sepcification.
%
This is the approach taken in~\cite{DBLP:conf/fsttcs/BrazdilHKKR12} where no specification is considered. However, there is a catch. This construction is only correct under the assumption of~\cite{DBLP:conf/fsttcs/BrazdilHKKR12} that there are no states of $\imc$ with both external and internal transitions available.

\begin{example}
Consider the IMC $\imc$ on the left and the completely liberal specification on the right. Note that there are both internal and external actions available in $\mathsf{no}$.

\begin{tikzpicture}[node distance=1.4cm, outer sep=2,/tikz/initial text=,->,font=\scriptsize]
\node[state,initial] (5) {$\mathsf{i}$};
\node[state] (0) [right of=5] {$\mathsf{?}$};
%\node[state] (0) [below right of=5] {$\mathsf{?}$};
\node[state] (1) at ($(0)+(1.4,0.7)$) {$\mathsf{yes}$};
\node[state] (2) [below of=1] {$\mathsf{no}$};
\node[state,accepting] (4) [right of=1] {$\mathsf{win}$};
\node[state] (3) [right of=2] {$\mathsf{fail}$};
\path  (5) edge node[auto] {$\lambda$} (0) 
         (1) edge node[auto] {$\mathsf{a}$} (4)
         (0) edge node[auto,swap] {$\tau$} (2)
         (0) edge node[auto] {$\tau$} (1)
         (2) edge node[auto,swap,below right=-3.5] {$\tau$} (4)
         (2) edge node[auto,swap] {$\mathsf{a}$} (3);
%\node  [font=\large] at (0,0.9) {$\imc_\mathit{imperfect}$};
\end{tikzpicture}
~
\begin{tikzpicture}[node distance=1.2cm, outer sep=2,/tikz/initial text=,->,font=\scriptsize]
\node[state,initial] (s) {q};
\path  (s) edge[loop above, densely dashed] node[above] {$\mathsf{a}$} (s);
\end{tikzpicture}

\noindent
As $\tau$ transitions take zero time, the environment must spend almost all the time in states without $\tau$.
Hence, when $\mathsf{?}$ is entered, $\env$ is almost surely in such a state $e$. In $e$, action $\mathsf{a}$ either \emph{is} or \emph{is not} available. As there are no $\tau$ transitions available, the environment cannot change its state while $\mathsf{yes}$ or $\mathsf{no}$ are entered. Therefore, if $\mathsf{yes}$ is entered and $\mathsf{a}$ was available in $e$, the $\mathsf{a}$ transition to $\mathsf{win}$ has to be taken. Similarly, if the scheduler of $\imc$ decides to move to $\mathsf{no}$ and there was no $\mathsf{a}$ available in $e$, it cannot be taken now, and $\tau$ to $\mathsf{win}$ must be taken.

All in all, the environment \emph{``commits'' in advance} to synchronize either in both $\mathsf{yes}$ and $\mathsf{no}$ or in none of them. Therefore, in the game we define, $\playerenv$ cannot completely freely choose which external transition is/is not taken.
% 
Further, note that the scheduler $\sigma$ cannot observe whether $\mathsf{a}$ is currently available in $\env$, which intrinsically induces imperfect information.
\end{example}

Altogether, states of the arena of $\game$ are of the form $(c,q,t,A)\in C\times Q \times \Rset \times 2^{\actnotau}$ and represent the following information: $c$ and $q$ are the current states of the IMC $\imc$ and the specification $\spec$, respectively; $t$ is the time left before taking the timed transition in $\spec$; $A$ are the actions the environment is currently committed to, i.e.~must synchronize with if possible. The synchronization is also restricted by $q$, 
%we define $\actnotau(q):=
%\{B\subseteq \actnotau\mid \text{if $b\in B$ then $q\may{b}$; and if $q\must{b}$ then $b\in B$}\}$ 
it will always hold that $\{a\mid q\must{a}\}\subseteq A\subseteq\{a\mid q\may{a}\}$, denoted $A\models q$.

The game $\game$ in state $v_n=(c,q,t,A)$ at time $t_n$ is played as follows: in each round either the time bound in the specification is reached, or a Markovian transition occurs, or a non-Markovian transition occurs. Formally:
\begin{itemize}
\item If $t_n\neq t_{n-1}$ and \todo{T}
\begin{itemize}
 \item either $t\geq 0$ and $q\timetran{\leq d}q'$,
 \item or $t\leq 0$ and $q\timetran{\geq d}q'$,
 \item or $t=0$ and $q\timetran{=d}q'$,
\end{itemize}
then $\playerenv$ may choose to immediately ($t_{n+1}=t_n$) move to a state $v_{n+1}:=(c,q',t',A')$ where $t'$ is chosen randomly according to distribution $d'$ with $q\timetran{\bowtie d'}$\todo{T again} and $\playerenv$ chooses $A'$. 

It is the responsibility of $\playerenv$ never to enter a state with $t<0$ if $q\timetran{\leq d}$ or $q\timetran{= d}$ (if he does so, he loses). Similarly, he must preserve $A\models q$ at all times or he loses.
\item Otherwise, if there is no $a\in A\cup\{\tau\}$ with $c\acttran{a}$, $\playerenv$ chooses a delay $d>0$. Then Markovian transitions (if available) are resolved by randomly choosing a target state $c' $ and a time $m$ according to the distributions in $\imc$. Then $t_{n+1}:=t_n+\min\{d,m\}$ and
\begin{itemize}
 \item if $m<d$ then the game moves to $v_{n+1}:=(c',q,t-m,A)$ 
 \item else ($d<m$) the game moves to $v_{n+1}:=(c,q,t-d,A')$ with $\playerenv$ choosing $A'$
\end{itemize}
\item Otherwise, $\playercon$ chooses a probability distribution over $\tau$-successors of $c$ (if there are any). Then, $\playerenv$ either approves this choice (provided $\tau$ is available), $c'$ is chosen randomly according to this distribution and the game moves to $v_{n+1}:=(c',q,t,A)$. Or $\playerenv$ may reject this choice provided $a\in A$ is available and choose an $a$-successor $c'$ and a new $A'$ and the game moves to $v_{n+1}:=(c',q',t,A')$ where $q\may{a}q'$ and $\playerenv$ chooses $A'$. In both cases  $t_{n+1}:=t_{n}$.
\end{itemize}
This generates a run $v_0 t_1 v_1 t_1\cdots$. The set $(\arena\times \Rsetpo)^\ast\times \arena$ of prefixes of runs is denoted $\paths(\game)$.


We formalize the choice
of $\playercon$ as a \emph{strategy} $\sigma: \paths(\game) \rightarrow
\dist(\arena)$ and the choice of $\playerenv$ as a \emph{strategy} 
$\pi:\paths(\game) \rightarrow \arena\cup\Rsetp$.
We denote by $\Sigma$ and $\Pi$ the sets of all strategies of the players $\playercon$ and $\playerenv$, respectively. 

Since $\playercon$ is not supposed to observe the state of the specification and the state of $\commit$, 
% Further, to keep the correspondence of a strategy $\sigma$ and a scheduler $\sigma\in\scheduler(\closedspec)$, 
we consider in $\Sigma$ only those strategies that satisfy $\sigma(p)=\sigma(p')$, whenever \emph{observations} of $p$ and $p'$ are the same. Like before, the observation of $(c_0,q_0,e_0)t_1\cdots t_{n}(c_n,q_n,e_n)\in\paths(\game)$ is a sequence obtained from $c_0t_1\cdots t_{n}c_n$ by replacing each maximal consecutive sequence $t_i\,c_i\cdots t_j\,c_j$ with all $c_k$ the same, by $t_i\,c_i$. This replacement takes place so that the player cannot observe transitions that do not affect $\imc$. Notice that now $\scheduler(\imc)$ is in one-to-one correspondence with $\Pi$.
Further, in order to keep CE games out of Zeno behaviour, we consider in $\Pi$ only those strategies 
for which the induced Zeno runs have zero measure, i.e.\ the sum of the chosen
delays diverges almost surely no matter what $\playercon$ is doing.

We now show that the value of $\game$ coincides with the value of compositional time-bounded reachability conditioned by $\spec$.

\newcommand{\theoremcegamesok}{
Let $\probm^{\sigma, \pi}_\game\big[\reach^{\leq T}\goal'\big]$ be the probability of all runs of $\game$ induced by $\sigma$ and $\pi$ and reaching a state with the first component in $\goal$ before time $T$. Then
$$\sup_{\sigma \in \Sigma} \inf_{\pi \in \Pi} \probm^{\sigma, \pi}_\game\big[\reach^{\leq T}\goal'\big]
=
\sup_{\sigma\in\scheduler(\imc)} \inf_{\substack{\env\in \ENV: \env\models\spec\\
      \pi\in\scheduler(\closed, \sigma)}}
  \probm^{\pi}_{\closed}\big[\reach^{\leq T}\goal_\env\big]
$$ %\myspace\myspace
}
\begin{theorem}\label{thm:ceg}
\theoremcegamesok
\end{theorem}
% \begin{proof}[Proof Idea]
% ``$\leq$'': We can simulate every $\env$ and scheduler $\pi$ by a strategy of $\playerenv$. The random waiting of $\env$ determined by occurrence of \emph{Markovian} transitions could be simulated by $\playerenv$ if he were allowed to choose the delays \emph{randomly}. We show how to derandomize his strategy. Further, in each state of $\env$ only some external actions are available and $\playerenv$ simulates this by changing the commitment to exactly this set of actions.
% 
% ``$\geq$'': Every strategy of $\playerenv$ can be (approximately) implemented using a suitable environment $\env$ together with a scheduler $\pi$. We need to simulate the discrete delays chosen by $\playerenv$ using random delays available in $\env$. A delay $t$ is simulated by many repetitions of a special Markovian transition with a very fast rate $\lambda$. After the total time adds up to at least $t$, $\pi$ stops repeating it and continues simulating the discrete transitions of $\playerenv$. We get the result by taking $\lambda \to \infty$.
% \end{proof}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> intro.tex <==
% $Id: intro.tex 341 2012-10-09 13:11:50Z xkretins $

\section{Introduction}

The ever increasing complexity and size of systems together with software reuse strategies  naturally enforce the need for component based system development. For the same reasons, checking reliabililty and optimizing performance of such systems needs to be done in a \emph{compositional} way. Since the systems are too large to be analyzed in their entirety, one prefers to check individual guarantees for each component in isolation, so as to derive a global system guarantee from the individual component guarantees. The key to getting useful guarantees is to consider each component in combination with assumptions on its context. The context is  usually the environment, consisting of the other components and their interaction. The assumptions can be refined in an iterative process, where guarantees obtained for one component turn into environmental assumptions for another. This \emph{assume-guarantee reasoning} is arguably a successful divide-and-conquer technique in many contexts~\cite{DBLP:journals/tse/MisraC81,DBLP:conf/lics/AlurH96,DBLP:conf/concur/AlurH97,DBLP:conf/hybrid/HenzingerMP01}. In many typical scenarios however, the environment of a component might be entirely or partially unknown. Either it must be assumed to behave completely hostile or only an abstract specification is at hand, for instance provided as part of a service-oriented architecture. 
In these circumstances, the analysis of the entire system is not only practically infeasible, but simply impossible. \todo{HH: don't like this last sentence.}

Compositional analyses of correctness and performance properties are not limited to deterministic systems. On the one hand, one can strive for synthesizing strategies (schedulers) for non-deterministic components that \emph{optimize} guarantees on performance. 
On the other hand, one may strive for the  analysis and optimisation of \emph{probabilistic and timed} systems. In this work, we combine both and consider strategy synthesis for continuous-time stochastic systems, namely interactive Markov chains.

\smallskip

\textbf{Interactive Markov chains} (IMC) are behavioral models of probabilistic systems running in continuous real time appropriate for the component-based approach~\cite{fmco09,Her02a,Bra06}.
IMC have a well-understood compositional theory, rooted in process algebra~\cite{BePS01}, and are in use as semantic backbones for dynamic fault trees~\cite{Bou10}, architectural description languages~\cite{arcade,esa10}, generalized stochastic Petri nets~\cite{HKNZ10} and Statemate~\cite{Boe09} extensions, and are applied in a large spectrum of practical applications, ranging from
networked hardware on chips~\cite{Cos09} to water treatment facilities~\cite{water} and ultra-modern satellite
designs~\cite{jpk-icse12}.

IMC arise from classical labeled transition systems by incorporating the possibility to change state according to a random \emph{delay} governed by a negative exponential distribution. 
By dropping the delay transitions, labeled transition systems are regained in their entirety. Dropping
action-labeled transitions instead yields continuous-time Markov chains -- one of the most used performance models.
In IMC, state transitions may be triggered by delay expirations, or may be triggered by the execution of \emph{internal} ($\tau$) actions or \emph{external} (synchronization) actions. Internal actions are assumed to happen instantaneously and therefore take precedence over delay transitions.
% while external actions do not. % Krc
External actions are the process algebraic means for interaction with other components. 

The fundamental problem in the analysis of IMC, akin to problems of paramount importance in many general real-time systems, is that of \emph{time-bounded reachability}. It is the problem to approximate the probability that a given set of states is reached within a given deadline. We illustrate the compositional setting of this problem in the following examples. \todo{Krc: change the sizes of lables in states at least to footnotesize, preferably small}

\smallskip

\begin{wrapfigure}{r}{0.27\textwidth}
\vspace*{-1.3em}
\begin{tikzpicture}[x=1.7cm,->,>=stealth',
% state style
state/.style={shape=circle,draw,font=\scriptsize,inner sep=1mm,outer sep=0.8mm, minimum size=0.75cm},
branch/.style={shape=circle,draw,inner sep=0.5mm,thick,outer sep=0.8mm},
multiline/.style={text width=12mm,text centered},
% target state
target/.style={double distance=0.2mm},
% probability style
transition/.style={},
rate/.style={above,color=black,font=\scriptsize},
tau/.style={rate,color=blue,font=\large},
prob/.style={rate,color=black},
]

\node[state] (X) {$\mathit{init}$};
\node[state] (Y) at (1,1) {$s$};
\node[state] (Y') at (1,0) {$t$};
\node[state] (Y'') at (1,-1) {$u$};
\node[state] (Z) at (2,0) {$\mathit{goal}$};

\path ($(X)+(-0.5,0)$) 		edge [transition]		(X);
\path[->] (X) edge node[above]{$a$} (Y); 
\path[->] (X) edge node[below]{$\tau$} (Y');
\path[->] (X) edge node[below]{$\tau$} (Y'');
\path[->] (Y) edge node[above]{$2$} (Z);
\path[->] (Y') edge node[below]{$1$} (Z);
\path[->] (Y'') edge node[below]{$3$} (Z);
\end{tikzpicture}
\vspace*{-1.2em}
\end{wrapfigure}
\textbf{Example.} Consider the IMC $\imc$ on the right to be composed with an unknown IMC environment $\env$. Either $\env$ is initially not ready  to synchronize on the external action $a$ and thus one of the internal actions is taken, or $\env$ is indeed willing to synchronize on $a$ at initialisation time. In the latter case, the choice is resolved non-determinstically. Since this is out of control  of $\imc$, we must assume the worst case and let the environment decide which of the two options will happen. For more details on this design choice, see~\cite{DBLP:conf/fsttcs/BrazdilHKKR12}. If $a$ were selected by the environment, the probability to reach $\mathit{goal}$ within time $t=1.5$ is $1-e^{2t}\approx0.95$. Otherwise, $\imc$ is given the choice to move to $t$ or $u$. Naturally, the choice maximizing the chance to get to $\mathit{goal}$ on time is $u$ as it has a higher rate associated. In this case the probability amounts to  $1-e^{t}\approx0.99$, while if $t$ were chosen, it would be only $0.78$. Altogether, the 
guaranteed probability is $95\%$ and the strategy of $\imc$ is to choose $u$ in $\mathit{init}$.

%\begin{wrapfigure}{r}{0.5\textwidth}
\begin{figure}

\vspace*{-2em}
\end{figure}
%\end{wrapfigure}
\todo{The pic here could have the same node layout than the previous, to use wrapfig}
The following example illustrates the necessity of assumptions on the environment: 
%Without any assumptions 
As it is, the environment can drive the component to state $\mathit{ret}$  and let it get stuck there by not  synchronising on $\mathsf{req}$ ever. Hence no better guarantee than $0$ can be derived. However, let us now assume that once synchronization on $\mathsf{req}$ occurs, the environment will be ready to synchronise on $\mathsf{resp}$ within some random time according to, say, an exponential distribution with rate $2$. Under this assumption, we are able to  derive a guarantee of $95\%$, just as in the previous example.

\begin{center}

\begin{tikzpicture}[x=1.7cm,->,>=stealth',
% state style
state/.style={shape=circle,draw,font=\scriptsize,inner sep=1mm,outer sep=0.8mm, minimum size=0.75cm},
branch/.style={shape=circle,draw,inner sep=0.5mm,thick,outer sep=0.8mm},
multiline/.style={text width=12mm,text centered},
% target state
target/.style={double distance=0.2mm},
% probability style
transition/.style={},
rate/.style={above,color=black,font=\scriptsize},
tau/.style={rate,color=blue,font=\large},
prob/.style={rate,color=black},
]

\node[state] (X) {$\mathit{init}$};
\node[state] (Y) at (1,0) {$\mathit{proc}$};
\node[state] (Y') at (2,0) {$\mathit{ret}$};
\node[state] (Z) at (3,0) {$\mathit{goal}$};

\path ($(X)+(-0.5,0)$) 		edge [transition]		(X);
\path[->] (X) edge node[above]{$\mathsf{req}$} (Y); 
\path[->] (Y) edge node[above]{$\tau$} (Y');
\path[->] (Y') edge node[above]{$\mathsf{resp}$} (Z);
\path[->] (X) edge[bend right] node[below]{$\tau$} (Z);
\end{tikzpicture}
 \vspace*{-0.7em}
\end{center}


Observe the form of the time constraint we imposed in the last example: ``within a random time distributed according to Exp(2)'' or symbolically $\Diamond_{\leq Exp(2)}\varphi$. We call this a \emph{continuous time constraint}. If a part of the environment is e.g.~a model of a network, it is clear we cannot impose hard bounds (discrete time constraints) such as ``within 1.5'' as in e.g.~a formula of MTL $\Diamond_{\leq 1.5}\varphi$. Indeed, the packets can get lost on the way for longer than that. Yet we want to express high assurance that they get there on time. Of course, in this case one might use e.g.~a formula of CSL $Pr_{\geq0.95}(\Diamond_{\leq 1.5}\varphi)$. However, when considering sequential composition of delay transitions as in $\mathit{init}\tran{2}s\tran{3}\mathit{goal}$ it is not clear which combination of time bounds and probabilities we should ask for. Moreover, we get more precise results by knowing all combinations, which corresponds to the information about the whole distribution. 
%Further, to cover operators like $Pr_{\geq0.95}$, we can consider subdistributions.

\smallskip

\textbf{Our contribution} is the following:
% \begin{itemize} % Jena: pak se odkazujes k ``second point''
\begin{enumerate}
 \item We introduce the first specification framework for IMC, illustrate its usabililty and argue for its completeness with respect to time-bounded reachability.
 \item We show how to synthesize $\varepsilon$-optimal schedulers for IMC in an unknown environment and approximate the resulting guarantee.% in polynomial time.
 \item We incorporate the assume-guarantee reasoning to the framework. We show how to synthesize $\epsilon$-optimal schedulers for IMC in an \emph{unknown environment satisfying a given specification} and again approximate the respective guarantee.% in polynomial time.
% \end{itemize}
\end{enumerate}

The specification framework we suggest is a behavioural one as we find it very intuitive. In essence, we extend timed automata with modalities and continuous-time constraints. 

In our recent work~\cite{DBLP:conf/fsttcs/BrazdilHKKR12} we consider a very restricted setting of the second point, where the given IMC component never enables internal and external transitions at the same state. This was a severe limitation as this property is not preserved during the IMC composition process and restricts the expressivity significantly. Both examples above violate this assumption. In this paper, we lift the assumption. Technically, this shifts the solution methods from complete information stochastic games to \emph{partial observation} stochastic games, where we need to solve the quantitative reachability problem. Note that quantitative reachability is undecidable for such games in general due to~\cite{Paz:1971} (and even the qualitative reachability problems are EXPTIME-complete~\cite{DBLP:conf/stoc/Reif79,DBLP:conf/csl/ChatterjeeDHR06}). However, we reduce our problem to a game played on an acyclic graph (where the qualitative reachability is easier, namely PSPACE-complete~\cite{DBLP:conf/lpar/ChatterjeeD10}). As to the quantitative reachability in the acyclic case, the folklore result is to encode it into the theory of reals, yielding an EXPSPACE algorithm due to~\cite{DBLP:journals/jcss/Ben-OrKR86}.
We show that for our game the quantitative reachability is in EXPTIME.

% Although partial observation these are lot more complicated, we show that this class can be solved in polynomial time as opposed to the general PSPACE-complete case. The class of games we introduce is interesting in its own right since it allows for modelling continuous-time components in an environment which can delay communication both in a probabilistic and non-deterministic way.
% 
% \todo{co time-bounded ``properties''? chceme neco obecnejsiho jako csl...?}

\smallskip

\textbf{Related work.}
The \emph{synthesis} problem is often stated as a game where the first player controls a component and the second player simulates an environment~\cite{ramadge1989}. Model checking of \emph{open} systems, i.e.~operating in an unknown environment, has been proposed in~\cite{KV_CAV_96}. There is a body of work on \emph{assume-guarantee} reasoning for parallel composition of \emph{real-time} time systems~\cite{DBLP:conf/concur/TasiranAKB96,DBLP:conf/concur/AlurH97,DBLP:conf/hybrid/HenzingerMP01}. Lately, games with \emph{stochastic continuous-time} have gained attention~\cite{DBLP:conf/icalp/BouyerF09,DBLP:journals/acta/RabeS11,Bra09,DBLP:conf/concur/BrazdilKKKR10}. While the second player models possible schedulers of the environment, the structure of the environment is fixed there and the verification is thus not compositional. The same holds for~\cite{DBLP:conf/qest/Sproston11,DBLP:conf/qest/HahnNPWZ11}, where time is under the control of the components.

A compositional framework requires means for specification of systems. A specification can be also viewed as an \emph{abstraction} of a set of systems. Three valued abstractions stemming from~\cite{DBLP:conf/lics/LarsenT88} have also been applied to the timed setting, namely in~\cite{DBLP:conf/cav/KatoenKLW07} to continuous-time Markov chains (IMC with no non-determinism), or in~\cite{DBLP:conf/formats/KatoenKN09} to IMC. Nevertheless, these abstractions do not allow for constraints on time distributions. Instead they would employ abstractions on transition probabilities. Further, a compositional framework with timed specifications is presented in~\cite{DBLP:journals/sttt/DavidLLMNRSW12}. This framework explicitely allows for time constraints. However, since the systems under consideration have non-detrministic flow of time (not stochastic), the natural choice was to only allow for discrete (not continuous) time constraints.

Although IMC support compositional design very well, analysis techniques for IMC proposed so far~\cite{cadp,mrmc,conf/mmb/HermannsJ08,Kat09b,Neu10,imca} are not compositional. They are all bound to the assumption that the analyzed IMC is a \emph{closed} system, i.e.\ it does not depend on interaction with the environment (all actions are internal). Some preliminary steps to develop a framework for synthesis of controllers based on models of hardware and control requirements have been taken in~\cite{DBLP:conf/acsd/Markovski11}. The first attempt at compositionality is our very recent work~\cite{DBLP:conf/fsttcs/BrazdilHKKR12} discussed above. 

The \emph{time-bounded reachability} problem for closed IMC has been studied and algorithms to compute it have been given
in~\cite{conf/mmb/HermannsJ08,Neu10,buchholz-schulz11,HH13} and compositional
abstraction techniques to compute it are developed in~\cite{Kat09b}. In the closed interpretation,
IMC have some similarities with continuous-time Markov decision
processes, CTMDP.  Algorithms for time-bounded reachability in
CTMDP and corresponding games are developed
in~\cite{Bai05b,Bra09,DBLP:journals/acta/RabeS11,buchholz-schulz11}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> other.tex <==
\section{Temporarily left out}

The pivotal problem in the  algorithmic analysis of IMC is to compute this value
together with a scheduler that achieves the supremum. As the value is not
rational in most cases, the aim is to provide an efficient approximation
algorithm and compute an $\varepsilon$-optimal scheduler.  The value of time-bounded reachability can be
approximated up to a given error tolerance $\varepsilon>0$ in time
$\mathcal{O}(|\states|^2\cdot (\lambda T)^2/\eps)$~%
%page 139 in \cite{Neuhauser:PhD}
\cite{Neuhauser:PhD}, where $\lambda$ is the
maximal rate of $\imc$, and the procedure also yields an
$\varepsilon$-optimal scheduler. We generalize both the notion of the value
as well as approximation algorithms to the setting of \emph{open} IMC,
i.e. those that are not closed, and motivate this extension in the next
section.

---------------------------------------------------

% \subsection{Behaviours of environments}
% 
% We define a probability space $\mathcal P_{\imc,\sigma,\env,\pi}$ as a projection of $\mathcal P_{\closed,\pi}$ onto in the observable information about the environment as follows: (co-inductively)\todo{dostat $a$ determinsiticky z prechodu - vytvorit jedinecne stavy?}
% \[
% p(s_n t_n s_{n+1} t_{n+1} \rho)=
% \begin{cases}
% E(s_n)\ a\ p(s_{n+1} t_{n+1} \rho) & \text{if $a:=\pi(s_0\cdots s_n)$ is synchronization}\\ 
% E(s_n)\ t_n\ p(s_{n+1} t_{n+1} \rho) & \text{else if $E(s_n)\neq E(s_{n+1})$}\\ 
% p(s_n\ t_n+t_{n+1}\ \rho) & \text{else}
% \end{cases}
% \]
% where $E((c,e))=\{a\in\actnotau\mid e\acttran{a}\}$ are the action currently enabled for synchronization by the environment. Intuitively, we only record when the environment changes on which channels it wants to synchronize or when it indeed synchronizes.
% 
% \begin{definition}[Semantics of environments]
% (For a closed IMC $\imc$, we define $\semantics{\imc}=\{\mathcal P_{\imc,\sigma}\mid \sigma\in\scheduler(\imc)\}$.)
% For an open IMC $\env$, we define $\semantics{\env}=\{\mathcal P_{\imc,\sigma,\env,\pi} \mid \imc\in\IMC,\sigma\in\scheduler(\imc),\pi\in\scheduler(\closed,\sigma)\}$.
% \end{definition}

---------------------------------------------------------

In this section we turn our attention to the central questions studied in this paper. How
can we decide how well an IMC component $\imc$ performs (w.r.t.\
time-bounded reachability) when acting in parallel with an unknown
environment? And how to control the component to establish a guarantee
as high as possible? 

Speaking thus far in vague terms, this amounts to finding a
scheduler %controller
$\sigma$ for $\imc$ which maximizes the probability of reaching a target set
$G$ before $T$ no matter what environment $\env$ is composed with $\imc$. As
we are interested in compositional modeling using IMC, the environments are
supposed to be IMC with the same external actions as $\imc$ (thus resolving
the external non-determinism of $\imc$). We also need to consider all
resolutions of the internal non-determinism of $\env$ as well as the
non-determinism arising from synchronization of $\imc$ and $\env$ using
another scheduler $\pi$.  So we are interested in the following value:
$$\sup_\sigma\inf_{\substack{\env,\pi}} \probm[\text{$G$ is reached in
composition of $\imc$ and $\env$ before $T$ using $\sigma$ and
$\pi$}].$$ 
%\todo{This intuition currently differs from the formal definition, don't have a suitable version though :-(}

%In what follows we make this intuition precise.
%In what follows we introduce the concept formally.
Now, let us be more formal and fix an IMC
$\imc=(\states,\act,\mathord{\itran},\mathord{\mtran},\init)$.  For a given
environment IMC $\env$ with the same action alphabet $\act$, we introduce a
composition
$$\closed = (\imc\comp{\actnotau}\env)\hide{\actnotau }$$%\quad 
where all open actions are hidden, yielding a closed system.  
Note that the states of $\closed$ are pairs $(c,e)$ where
  $c$ is a state of $\imc$ and $e$ is a state of $\env$.
%Contrary to
%the time-bounded reachability, we consider two schedulers here. 
We consider a
scheduler $\sigma$ of $\imc$ %, called \emph{controller}, 
and a scheduler $\pi$ of $\closed$ respecting $\sigma$ on internal
actions of $\imc$.
% Formally, we write $\pi\in\scheduler(\closed, \sigma)$
% to state that $\pi\in\scheduler(\closed)$ and for any path
% $\history=(c_0,e_0)\,t_0\cdots t_{n-1}(c_n,e_n)\in\paths(\closed)$ and its
% first projection \todo{$\sigma$ sees the time stamps of all intermediate
%   steps of $\env$, but do we care?  Total Time Positional anyway - maybe
%   footnote.}$\history_\imc=c_0t_0\cdots c_nt_n$, it holds that
% %  \[
% % \pi(\history) \in \{ (c,e)  \mid
% % \mbox{ either }
% % c_n\acttran{a}c \mbox{ and }e_n\acttran{a}e \mbox{, or }
% % c_n=c \mbox{ and } e_n\acttran{\tau}e \} \cup  \{ (\sigma(\history_\imc),e_n) \}.
% % \]
% %\todo{or the following formulation}
%  \[
% \pi(\history) \in 
% \{ (c,e)  \mid c_n\acttran{a}c \mbox{ and }e_n\acttran{a}e \}\cup
% \{ (c_n,e)  \mid e_n\acttran{\tau}e \} \cup 
% \{ (\sigma(\history_\imc),e_n) \}.
% \]
% %
We say that $\pi$ {\em respects $\sigma$}, % on $\imc$}
denoted by $\pi\in\scheduler(\closed, \sigma)$, if for every
history
$\history=(c_0,e_0)\,t_0\cdots
t_{n-1}(c_n,e_n)$ of $\closed$ the scheduler $\pi$ satisfies one of
the following conditions:
\begin{itemize}
\item $\pi(\history)=(c,e)$ where $c_n\acttran{a}c$ and $e_n\acttran{a}e$
  \quad {(\footnotesize $\pi$ resolves synchronization)}
\item $\pi(\history)=(c_n,e)$ where $e_n\acttran{\tau}e$ \quad
  {(\footnotesize $\pi$ chooses a move in the environment)}
\item $\pi(\history)=(\sigma(\history_\imc),e_n)$ where $\history_\imc=c_0
  t_0\cdots t_{n-1} c_n$ \quad {(\footnotesize $\pi$ chooses a move in $\imc$
    according to $\sigma$)}.% \todo{$\sigma$ sees the time stamps of all
    % intermediate steps of $\env$, but do we care?  Total Time Positional
    % anyway - maybe footnote.}
\end{itemize}


%\todo{other formulations are commented in the source code}
%\todo{or the following formulation}
%  \[
% \pi(\history)=
% \begin{cases}
% (c,e) & \mbox{if either }
% c_n\acttran{a}c \mbox{ and }e_n\acttran{a}e \mbox{, or }
% c_n=c \mbox{ and } e_n\acttran{\tau}e  \\
% (\sigma(\history_\imc),e_n) & \mbox{otherwise, i.e.\ if only an internal $\tau$
%   transition of $\imc$ is chosen.} %c_n\acttran{\tau}c \mbox{ and } e_n=e
% \end{cases}
% \]
% \todo{Krc: the two cases are still not disjunct; we can have $c_n
%   \acttran{a} c$, $e_n \acttran{a} e$ as well as $c_n \acttran{\tau} c$,
%   $e_n = e$. VR: Solution is to add only.}

%The value of our interest is stated as follows. 
Given % an  \emph{closed} IMC
      % $\imc=(\states,\act,\mathord{\itran},\mathord{\mtran},\init)$, 
a set of goal states $\goal\subseteq\states$ and a time bound $T\in\Rsetpo$,
the \emph{value of compositional time-bounded reachability} is defined as
\begin{align*}
& &
\sup_{\sigma\in\scheduler(\imc)} \inf_{\substack{\env\in \ENV\\
      \pi\in\scheduler(\closed, \sigma)}}
  \probm^{\pi}_{\closed}\big[\reach^{\leq T}\goal_\env\big] \tag{$*$}
\end{align*}
where $\ENV$ denotes the set of all IMC with the action alphabet $\act$ and
$\goal_\env =\goal \times \states_\env$ where $\states_\env$ is the set of
states of $\env$.  As for the closed IMC, our goal is to efficiently
approximate this value together with a maximizing scheduler. 



\begin{assumpt}
\label{ass:B}
Each cycle %in an IMC 
contains a Markovian transition.
% \todo{VR: Changed to a bit weaker assumption, confirmed by JKrc.}
%Each cycle in an IMC contains a state where only Markovian transitions are available.
\end{assumpt}
%\mytinyvspace
%
This assumption is standard over all analysis techniques published for
IMC~\cite{cadp,mrmc,conf/mmb/HermannsJ08,Kat09b,Neu10,imca}. It
implies that the probability of taking infinitely many transitions in
finite time, i.e. of Zeno behavior, is zero.  This is a rather natural assumption and does not restrict the modeling power much, since no 
real system will be able to take infinitely many transitions in
finite time anyway.  Furthermore, the assumed property is a compositional one,
i.e.  it is preserved by parallel composition and hiding. \todo{argumentovat ze CTMDP nebo PEPA nemaji ani dva kroky za sebou}


\begin{theorem}\label{thm:main}
% The problem of approximating the value $\valcomp$ up to $\eps$ and
% synthesizing an $\eps$-optimal scheduler for the IMC $\imc$ can be solved
% in time $\mathcal{O}(|S|^2\cdot (\lambda T)^2/\eps)$. 
  Let $\eps>0$ be an approximation bound and
  $\imc=(\states,\act,\mathord{\itran},\mathord{\mtran},\init)$ be an IMC
  satisfying Assumptions~\ref{ass:B} and \ref{ass:A}. Then one can
  approximate the value of compositional time-bounded reachability of $\imc$
  up to $\varepsilon$ and compute an $\eps$-optimal scheduler in time
  $\mathcal{O}(|\states|^2\cdot (\lambda T)^2/\eps)$, where $\lambda$ is the
  maximal rate of $\imc$ and $T$ is the reachability time-bound.
\end{theorem}
\noindent
%\todo{Sometimes the approximation theorems are stated in a more precise way: There is $x$ computable in time
%$\mathcal{O}(|\states|^2\cdot (\lambda T)^2/\eps)$ such that $|x-{value}|\leq \varepsilon$. I am suggesting this for discussion ....} 
%\todo{Krc: I am completely fine with this level of precision.}
In the remainder of the paper, we prove this theorem and discuss its
restrictions.  First, we introduce a new kind of real-time games, called CE
games, that are played on open IMC. Then we reduce the compositional
time-bounded reachability of $\imc$ to time-bounded reachability objective
in the CE game played just on the component $\imc$ (see
Proposition~\ref{thm:ce-games-ok}).  In Section~\ref{sec:disc}, we show how
to reduce, using discretization, the time-bounded reachability in CE games
to step-bounded reachability in discrete-time stochastic games (see
Proposition~\ref{thm:error-bound}), that in turn can be solved using simple
backward propagation.  Finally, we show, in
Proposition~\ref{thm:scheduler-synthesis}, how to transform optimal
strategies in the discretized stochastic games to $\eps$-optimal schedulers
for $\imc$.

==> pogames.tex <==
% \section{Acyclic Partially Observable Games}\label{sec:pog}

% For \emph{acyclic} games, the naive solution would be a reduction to the theory of reals, yielding an EXPSPACE algorithm. However, a much better option is to make use of the developed theory of \emph{extensive-form} games.

% We first take an unfold of the game up to $n$ steps. Such a game tree satisfies the \emph{perfect recall} condition, roughly meaning that none of the players ever forgets her own moves. For partially observable tree games with perfect recall, the result of~\cite{DBLP:conf/stoc/KollerMS94} can be applied.

% 
% Now for your question on acyclic games with quantitative reachability I guess the best complexity is through theory of reals. I am not sure if anyone has looked into it for a better complexity. I dont know of a explicit reference as I am not sure if anyone has explicitly stated this as a theorem in a paper. But as far I know you can say that naive way would be reduction to theory of reals, which may give something like a  EXPSPACE algorithm.
% 


==> tikz_discretization_without_title.tex <==
% $Id: tikz_discretization_without_title.tex 292 2012-07-13 11:57:19Z xkrcal4 $

\ifx\mainfile\undefined

\renewcommand{\Box}{Box}

\newcommand{\states}{S}
\newcommand{\ext}{e}
\newcommand{\Mar}{M}

\newcommand{\imc}{M}


\newcommand{\game}{\mathcal{G}}

\newcommand{\gamed}{\Delta}

\newcommand{\vertices}{V}

\newcommand{\nowtran}{\mathsf{\mathbf{Now}}}
\newcommand{\committran}{\mathsf{\mathbf{Change}}}

\newcommand{\prand}{\bigcirc}
\newcommand{\pmin}{GRR}
\newcommand{\pmax}{\Box}
\newcommand{\parb}{\odot}

\newcommand{\reachd}{\reach}
\newcommand{\steps}{\#_\text{\circle{3}}}
\newcommand{\stepsc}{\#_\imc}
\newcommand{\reachdn}{\reachd^{\steps\leq N}}

\newcommand{\vrand}{\vertices_\prand}
\newcommand{\vmax}{\vertices_\pmax}
\newcommand{\vmin}{\vertices_\pmin}
\newcommand{\varb}{\vertices_\odot}

\newcommand{\dprob}{Prob}
\newcommand{\dtran}{{\,\mapsto\,}}

\newcommand{\sucd}{\mathrm{succ}_{\dtran}}

\newcommand{\Sigmad}{\Sigma_\Delta}
\newcommand{\Pid}{\Pi_\Delta}

\newcommand{\markovianvalue}{\mathcal{A}}
\newcommand{\discretevalue}{\mathcal{B}}

\newcommand{\deltasteps}{\#_{[0,\delta]}}

\usetikzlibrary{arrows}
\usetikzlibrary{shapes}
\usetikzlibrary{automata}
\usetikzlibrary{decorations.pathmorphing} % for snake lines
\usetikzlibrary{decorations.pathreplacing} % for snake lines
\usetikzlibrary{calc} % for manimulation of coordinates


\newcommand{\todo}[1]{%
  % Add to todo list
  %
\vspace*{-1em}
  \begin{tikzpicture}[remember picture]%
      \node [coordinate] (inText) {};%
  \end{tikzpicture}%
  %
  % Make the margin par
  \marginpar{%
      \begin{tikzpicture}[remember picture]%
   %
          \draw node[draw=red, color=red, text width = 1cm] (inNote)%
                   {{\small #1}};%
      \end{tikzpicture}%
  }%
  %
  \begin{tikzpicture}[remember picture, overlay]%
      \draw[draw = red, thick]%
          ([yshift=-0.1cm] inText)%
              -| ([xshift=-0.1cm] inNote.west)%
              -| (inNote.west);%
  \end{tikzpicture}%
  %
}%


\fi
% 
\tikzstyle{snakeline} = [trans,thick, decorate, decoration={
						pre length=0.05cm,
                         post length=0.1cm, snake, amplitude=.2mm,
                         segment length=2mm},thick, trans]
% 
\tikzstyle{title} = []
% 
\tikzstyle{state} = [draw, circle, inner sep=0.1em, outer sep=0.1em,font=\footnotesize,scale=0.6]
\tikzstyle{box} = [state, rectangle, inner sep=0.2em,minimum size=1cm]
\tikzstyle{evil} = [state, diamond,inner sep=0.1em]
\tikzstyle{unknown} = [rectangle, inner sep=0.1em,font=\footnotesize,scale=0.6]
\tikzstyle{trans} = [->,sloped]
\tikzstyle{transnode} = [font=\footnotesize,->,scale=0.8]
\tikzstyle{trans_vertical} = [font=\tiny,->]
\tikzstyle{comment} = [font=\scriptsize,text width=10em,right]   %[font=\scriptsize,text width=10em,align=left,right]
% 
\begin{figure}[t]

\centering
% \hspace{-7.2em}
\begin{tikzpicture}[ x=2cm,y=2cm]

 \path[use as bounding box] (-0.27, -2.12) rectangle (5.67,0.45);

\node (title) at (0.35,0.8) {};
\node (prime) at (0,-1.5) {};
\node (snake) at (0.3,-0.5) {};
\node (snake') at (0.3,-0.9) {};
\node (snakecomment) at (0.4,-0.7) {};
\node (line) at (-0.7,0.7) {};
\node (line') at (-0.7,-2.4) {};

\node (master) at (0,0.4) {};
\node (slave) at (0,-0.4) {};

\node (narrow) at (0.65,0) {};
\node (wide) at (1,0) {};
\node (wider) at (1.2,0) {};

\node (col_narrow) at (2,0) {};
\node (col_wide) at (2.2,0) {};

\node (two_one) at (0,0.4) {};
\node (two_two) at (0,-0.4) {};

\node (four_one) at (0,0.375) {};
\node (four_two) at (0,0.125) {};
\node (four_three) at (0,-0.125) {};
\node (four_four) at (0,-0.375) {};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \node (one) at (0,0) {};
% \node (one') at ($(one)+(prime)$) {};
% 
% \node[state] (one_s) at ($(one)+(0,0)$) {$s$};
% \node[unknown] (one_s_1) at ($(one)+(narrow)+(two_one)$) {$s_1$};
% \node[unknown] (one_s_2) at ($(one)+(narrow)+(two_two)$) {$s_2$};
% 
% \path[trans] (one_s) edge node[auto] {$\tau$} (one_s_1);
% \path[trans] (one_s) edge node[auto,swap] {$\tau$} (one_s_2);
% 
% \draw [snakeline] ($(one)+(snake)$) -- ($(one)+(snake')$);
% 
% \node[box] (one'_s) at ($(one')+(0,0)$) {$s$};
% \node[unknown] (one'_s_1) at ($(one')+(narrow)+(two_one)$) {$s_1$};
% \node[unknown] (one'_s_2) at ($(one')+(narrow)+(two_two)$) {$s_2$};
% 
% \path[trans] (one'_s) edge node[auto] {} (one'_s_1);
% \path[trans] (one'_s) edge node[auto,swap] {} (one'_s_2);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node (two) at (0,0) {}; %($(one)+(col_narrow)$) {};
\node (two') at ($(two)+(prime)$) {};

\node[state] (two_s) at ($(two)+(0,0)$) {$(c,(q,t),e)$};
\node[unknown] (two_s_1) at ($(two)+(wide)+(four_one)$) {$(c_1,(q_1,t),e_1)$};
\node[unknown] (two_s_2) at ($(two)+(wide)+(four_two)$) {$(c_2,(q_2,t),e_2)$};
\node[unknown] (two_s_3) at ($(two)+(wide)+(four_three)$) {$(c_3,(q,t),e)$};
\node[unknown] (two_s_4) at ($(two)+(wide)+(four_four)$) {$(c_4,(q,t),e)$};

\path[trans] (two_s) edge node[transnode,auto,above=-3,pos=0.7] {$\tau$} (two_s_1.west);
\path[trans] (two_s) edge node[transnode,auto,above=-3,pos=0.7] {$\tau$} (two_s_2.west);
\path[trans] (two_s) edge node[transnode,auto,swap,below=-2,pos=0.7] {$\tau$} (two_s_3.west);
\path[trans] (two_s) edge node[transnode,auto,swap,below=-2,pos=0.7] {$\tau$} (two_s_4.west);

\draw [snakeline] ($(two)+(snake)$) -- ($(two)+(snake')$);
\node[comment] (two'_s) at ($(two)+(snakecomment)$) {$k = \lfloor t/\delta \rfloor$};
% \draw ($(two)+(line)$) -- ($(two)+(line')$);

\node[evil] (two'_s) at ($(two')+(master)$) {$(c,(q,k),e)$};
\node[box] (two'_sbar) at ($(two')+(slave)$) {$(\bar{c},(q,k),e)$};

\node[unknown] (two'_s_1) at ($(two')+(wide)+(four_one)$) {$(c_1,(q_1,k),e_1)$};
\node[unknown] (two'_s_2) at ($(two')+(wide)+(four_two)$) {$(c_2,(q_2,k),e_2)$};
\node[unknown] (two'_s_3) at ($(two')+(wide)+(four_three)$) {$(c_3,(q,k),e)$};
\node[unknown] (two'_s_4) at ($(two')+(wide)+(four_four)$) {$(c_4,(q,k),e)$};

\path[trans] (two'_s) edge node[transnode,auto] {} (two'_sbar);
\path[trans] (two'_sbar) edge node[transnode,auto,swap] {} (two'_s_3.west);
\path[trans] (two'_sbar) edge node[transnode,auto,swap] {} (two'_s_4.west);
\path[trans] (two'_s) edge node[transnode,auto] {} (two'_s_1.west);
\path[trans] (two'_s) edge node[transnode,auto] {} (two'_s_2.west);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% \node (four) at ($(two)+(col_wide)$) {};
% \node (four') at ($(four)+(prime)$) {};
% 
% \node[state] (four_s) at ($(four)+(0,0)$) {$s$};
% \node[unknown] (four_s_1) at ($(four)+(wide)+(two_one)$) {$s_1$};
% \node[unknown] (four_s_2) at ($(four)+(wide)+(two_two)$) {$s_2$};
% 
% \path[trans] (four_s) edge node[auto,pos=0.6] {$\lambda_1$} (four_s_1);
% \path[trans] (four_s) edge node[auto,swap,pos=0.6] {$\lambda_2$} (four_s_2);
% 
% \draw [snakeline] ($(four)+(snake)$) -- ($(four)+(snake')$);
% \draw ($(four)+(line)$) -- ($(four)+(line')$);
% 
% \node[state] (four'_s) at ($(four')+(0,0)$) {$s$} edge [trans,in=110,out=65,loop] node[auto,swap,pos=0.5] {$1-p$} ();
% \node[unknown] (four'_s_1) at ($(four')+(wide)+(two_one)$) {$s_1$};
% \node[unknown] (four'_s_2) at ($(four')+(wide)+(two_two)$) {$s_2$};
% 
% \path[trans] (four'_s) edge node[auto,pos=1.3] {$p.P(s,s_1)$} (four'_s_1);
% \path[trans] (four'_s) edge node[auto,swap,pos=1.1] {$p.P(s,s_2)$} (four'_s_2);


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\node (three) at ($(two)+(col_narrow)$) {};
\node (three') at ($(three)+(prime)$) {};

\node[state] (three_s) at ($(three)+(0,0)$) {$(c,(q,t),e)$};
\node[unknown] (three_s_1) at ($(three)+(wider)+(four_one)$) {$(c,(q,t),e_1)$};
%  \node[unknown] (three_s_2) at ($(three)+(wider)+(four_two)$) {$s_2$};
\node[unknown] (three_s_3) at ($(three)+(wider)+(four_three)$) {$(c_2,(q,t-x),e)$};
\node[unknown] (three_s_4) at ($(three)+(wider)+(four_four)$) {$(c_3,(q,t-x),e)$};

\path[trans] (three_s) edge node[transnode,auto,pos=0.7,above=-3] {$\lambda_1$} (three_s_3.west);
\path[trans] (three_s) edge node[transnode,auto,pos=0.7,above=-3] {$\lambda_2$} (three_s_4.west);
%  \path[trans] (three_s) edge node[auto,pos=0.6,above=-3,font=\footnotesize] {$\nowtran$} (three_s_2);
\path[trans] (three_s) edge node[transnode,above=-3,pos=0.6] {$\committran$} (three_s_1.west);

\draw [snakeline] ($(three)+(snake)$) -- ($(three)+(snake')$);
\node[comment] (three'_s) at ($(three)+(snakecomment)$) {$k = \lfloor t/\delta \rfloor$ \\ $p = 1-e^{-E((c,s,e))\cdot\delta}$};
% \draw ($(three)+(line)$) -- ($(three)+(line')$);

\node[evil] (three'_s) at ($(three')+(master)$) {$(c,(q,k),e)$};
\node[state] (three'_sbar) at ($(three')+(slave)$) {$(\bar{c},(q,k),e)$};

\node[unknown] (three'_s_1) at ($(three')+(wider)+(four_one)$) {$(c,(q,k),e_1)$};
\node[unknown] (three'_s_2) at ($(three')+(wider)+(four_two)$) {$(c,(q,k-1),e)$};
\node[unknown] (three'_s_3) at ($(three')+(wider)+(four_three)$) {$(c_2,(q,k-1),e)$};
\node[unknown] (three'_s_4) at ($(three')+(wider)+(four_four)$) {$(c_3,(q,k-1),e)$};

\path[trans] (three'_s) edge node[auto] {} (three'_sbar);
% \path[trans] (three'_sbar) edge node[auto,pos=1.13,font=\footnotesize] {$p.P(s,s_2)$} (three'_s_3);
% \path[trans] (three'_sbar) edge node[auto,swap,pos=0.6,font=\footnotesize] {$p.P(s,s_3)$} (three'_s_4);
\path[trans] (three'_sbar) edge node[transnode,auto,pos=0.9,rotate=3] {$p.\frac{\lambda_1}{\lambda_1+\lambda_2}$} (three'_s_3.west);
\path[trans] (three'_sbar) edge node[transnode,auto,swap,pos=0.6,rotate=-3,below=-2] {$p.\frac{\lambda_2}{\lambda_1+\lambda_2}$} (three'_s_4.west);
\path[trans_vertical,bend left=30] (three'_sbar) edge node[transnode,auto,pos=0.7,sloped] {$1-p$} (three'_s_2.west);
\path[trans] (three'_s) edge node[auto] {} (three'_s_1);
% \path[trans] (three'_s) edge node[auto] {} (three'_s_2);
%
% 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
\node (five) at ($(three)+(col_wide)$) {};
\node (five') at ($(five)+(prime)$) {};

\node[state] (five_s) at ($(five)+(0,0)$) {$(c,(q,0),e)$};
\node[unknown] (five_s_1) at ($(five)+(wider)+(four_one)$) {$(c,(q',0.15),e)$};
\node[unknown] (five_s_2) at ($(five)+(wider)+(four_two)$) {$(c,(q',0.49),e)$};
\node[unknown] (five_s_3) at ($(five)+(wider)+(four_three)$) {$(c,(q',0.68),e)$};

\path[trans] (five_s) edge node[auto,pos=0.85,swap,rotate=-15,below=-5] {$\vbox{\baselineskip=2pt \lineskiplimit=0pt \kern6pt \hbox{.}\hbox{.}\hbox{.}}$} (five_s_1.west);
\path[trans] (five_s) edge node[auto,pos=0.9,swap,rotate=-10,below=-5] {$\vbox{\baselineskip=2pt \lineskiplimit=0pt \kern6pt \hbox{.}\hbox{.}\hbox{.}}$} (five_s_2.west);
\path[trans] (five_s) edge node[auto,pos=0.9,swap,rotate=-0,below=-6] {$\vbox{\baselineskip=2pt \lineskiplimit=0pt 
\kern6pt \hbox{.}\hbox{.}\hbox{.}}$} (five_s_3.west);

\draw [snakeline] ($(five)+(snake)$) -- ($(five)+(snake')$);
\node[comment] at ($(five)+(snakecomment)$) {$p_i = F_{q'}(i \cdot\delta)$};
% \draw ($(five)+(line)$) -- ($(five)+(line')$);

\node[state] (five'_s) at ($(five')$) {$(c,(q,0),e)$};
\node[unknown] (five'_s_1) at ($(five')+(wider)+(four_one)$) {$(c,(q',1),e)$};
\node[unknown] (five'_s_2) at ($(five')+(wider)+(four_two)$) {$(c,(q',2),e)$};
\node[unknown] (five'_s_4) at ($(five')+(wider)+(four_four)$) {$(c,(q',N),e)$};

\path[trans] (five'_s) edge node[transnode,auto,pos=0.9] {$p_1-p_0$} (five'_s_1.west);
\path[trans] (five'_s) edge node[transnode,auto,pos=0.85,above=-2] {$p_2-p_1$} node[auto,pos=0.8,swap,rotate=-5] {$\vbox{\baselineskip=2pt \lineskiplimit=0pt \kern6pt \hbox{.}\hbox{.}\hbox{.}}$} (five'_s_2.west);
\path[trans] (five'_s) edge node[transnode,auto,pos=0.9,swap] {$p_N-p_{N-1}$} (five'_s_4.west);

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \node[rotate=90,font=\scriptsize] at ($(three')+(1.7,0)$)  {$p = 1-e^{-E((c,s,e))\cdot\delta}$};
% \draw [blue] (current bounding box.south west) rectangle (current bounding box.north east);

\end{tikzpicture}
% \vspace*{-1em}
\caption{Three gadgets for transforming immediate, timed, and resampling states of a CE game (above) into the discrete game (below).
% In the upper part, we label by $\tau'$ the transitions that correspond to internal transitions in $\imc$. 
% In the lower part, the square-shaped, diamond-shaped and circle-shaped vertices belong to players $\pmax$, $\pmin$ and to $\prand$, respectively. 
% Binary branching is displayed only in order to simplify the figure.
% 
% In immediate states on the left, $\pmin$ can either choose a $\tau$ transition not originating from $\imc$ or $\pmin$ can let $\pmax$ choose a $\tau$ transition of $\imc$.
In immediate states on the left, $\pmin$ can either let $\pmax$ choose a $\tau$ transition of $\imc$; or choose himself any other $\tau$ transition.
In timed states in the middle, $\pmin$ can either choose $\committran$ immediately or let the time flow by $\delta$ in the state of $\prand$ during which a Markovian transition is taken with probability $p$.
On the right, the continuous resampling is discretized into values $1$--$N$.
% 
}
\label{fig:discretization_w_t}
\end{figure}
